Understanding and Reusing Test Suites Across Database Systems

Database Management System (DBMS) developers have implemented extensive test suites to test their DBMSs. For example, the SQLite test suites contain over 92 million lines of code. Despite these extensive efforts, test suites are not systematically reused across DBMSs, leading to wasted effort. Integration is challenging, as test suites use various test case formats and rely on unstandardized test runner features. We present a unified test suite, SQuaLity, in which we integrated test cases from three widely-used DBMSs, SQLite, PostgreSQL, and DuckDB. In addition, we present an empirical study to determine the potential of reusing these systems' test suites. Our results indicate that reusing test suites is challenging: First, test formats and test runner commands vary widely; for example, SQLite has 4 test runner commands, while MySQL has 112 commands with additional features, to, for example, execute file operations or interact with a shell. Second, while some test suites contain mostly standard-compliant statements (e.g., 99% in SQLite), other test suites mostly test non-standardized functionality (e.g., 31% of statements in the PostgreSQL test suite are nonstandardized). Third, test reuse is complicated by various explicit and implicit dependencies, such as the need to set variables and configurations, certain test cases requiring extensions not present by default, and query results depending on specific clients. Despite the above findings, we have identified 3 crashes, 3 hangs, and multiple compatibility issues across four different DBMSs by executing test suites across DBMSs, indicating the benefits of reuse. Overall, this work represents the first step towards test-case reuse in the context of DBMSs, and we hope that it will inspire follow-up work on this important topic.

==> assets/table/PSQL-Error-Reasons.tex <==
\begin{table}
\centering
\caption{Number of errors for each reason}
\label{tab:psql-error-reasons}
\begin{tabular}{l|c}
\toprule
{} & Number of Errors \\
\midrule
ALREADYEXIST &                4 \\
COLLATION    &               47 \\
DEP-DDL      &               18 \\
DEP-DML      &                2 \\
DEP-EXT      &               37 \\
FUNCFORMAT   &                1 \\
LARGEOBJ     &               16 \\
NOEXIST      &              132 \\
Other        &               40 \\
PREPARETXN   &               20 \\
REGRESS      &               15 \\
SHOWTABLE    &               88 \\
TIMESTAMP    &               18 \\
\bottomrule
\end{tabular}
\end{table}


==> assets/table/RQ1-TestRunnerFeature.tex <==
\centering
\caption{Non-SQL commandTest Runner Features of each DBMS Test Runner}\label{table:RQ1-testrunner-feature}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ llccccc }
\toprule
& Feature & SQLite & MySQL & PostgreSQL &  DuckDB \\
\midrule
% \multirow{4}{*}{Test Case Format} &
% Record-like test case & \checkmark & - & - &  \checkmark \\ 
% &Whole file as test case & - & \checkmark & \checkmark & - \\ 
% &Row-wise results & - & \checkmark & \checkmark &  \checkmark \\ 
% &Value-wise results& \checkmark & - & - &  $\circ$ \\ 
% \midrule
% \multirow{10}{*}{Non-SQL Commands} &
% \texttt{echo} & - & \checkmark & \checkmark & - & - \\ 
Include & - & \checkmark & \checkmark &  - \\ 
&Set Variable & - & \checkmark & \checkmark &  \checkmark \\
&Load Database& - & \checkmark & \checkmark &  \checkmark \\
&Loop & - & \checkmark & - &  \checkmark \\ 
&Require External Dependency& - & - & \checkmark &  \checkmark\\
&Skiptest & \checkmark & - & - & \checkmark \\
&Sleep & - & \checkmark & - &  - \\
&Multi-ple Connections & - & \checkmark & \checkmark &  \checkmark \\
&CLI Commands & - & - & 59  & - \\ 
&Other Commands & 0 & 105 & 0 & 0 \\
\bottomrule
\end{tabular}

==> assets/table/RQ1-TestRunnerFeatureSingle.tex <==
\centering
\caption{Non-SQL commands of each DBMS Test Runner}\label{table:RQ1-testrunner-feature}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ lcccc}
\toprule
 Feature & SQLite & MySQL & PostgreSQL &  DuckDB \\
\midrule
% \multirow{4}{*}{Test Case Format} &
% Record-like test case & \checkmark & - & - &  \checkmark \\ 
% &Whole file as test case & - & \checkmark & \checkmark & - \\ 
% &Row-wise results & - & \checkmark & \checkmark &  \checkmark \\ 
% &Value-wise results& \checkmark & - & - &  $\circ$ \\ 
% \midrule
% \multirow{10}{*}{Non-SQL Commands} &
% \texttt{echo} & - & \checkmark & \checkmark & - & - \\ 
Include & - & \checkmark & \checkmark &  - \\ 
Set Variable & \checkmark & \checkmark & \checkmark &  \checkmark \\
Load Database& - & \checkmark & \checkmark &  \checkmark \\
Loop & - & \checkmark & - &  \checkmark \\ 
Require& - & - & \checkmark &  \checkmark\\
Skiptest & \checkmark & - & - & \checkmark \\
Sleep & - & \checkmark & - &  - \\
Multi-Connections & - & \checkmark & \checkmark &  \checkmark \\
CLI Commands & - & - & 59  & - \\ 
Other Commands & 0 & 105 & 0 & 0 \\
\bottomrule
\end{tabular}

==> assets/table/RQ3-ErrorReasons.tex <==
\begin{table*}[tb]
\centering
\caption{Number of errors for each reason}
\label{tab:rq3-error-reasons}
\begin{tabular}{ll|rrr}
\toprule
\multicolumn{2}{c|}{Error Type} & SQLite & DuckDB & PostgreSQL \\
\midrule
\multirow{3}{*}{Environment}&External     & 0 & &                52\\
&Locale Settings   & 0 & &               66 \\
&Transactions   & 0 & &              20 \\
\midrule
\multirow{2}{*}{Extension} & Shared Library & 0 & & \\
& External Tools & 0 & & \\
\midrule
\multirow{3}{*}{Runner} &Runner/Client Command   & 0 & &               104 \\
& Arithmetic & 2& & 0\\
& Engine & & & \\
\midrule
&Wrong Schema & 0 & &               156 \\
&Other        &  0&  &             40 \\
\bottomrule
\end{tabular}
\end{table*}

==> assets/table/RQ4-DuckDB-demo.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  SQLite &  PostgreSQL &  MySQL \\
\midrule
Unsupported SQL  &                  14\%  &     21\%       &        14\%    \\
Inconsistent Function  &                1\%  &       4\%     &        1\%    \\
Unsupported Function or Type  &       67\%  &      61\%      &         62\%     \\
Unsupported Operation &             18\% &     11\%    &        21\%   \\
Unsuccessful Setting &             0\%  &      2\%        &        1\%    \\
Misc                &               0\%  &        1\%       &         0\%   \\
\midrule
Crash & 0& 0& 1\\
\bottomrule
\end{tabular}


==> assets/table/RQ4-PGT-demo.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  SQLite &  DuckDB &  MySQL \\
\midrule
Unsupported SQL  &              34\%  &       29\%        &     32\%      \\
Inconsistent Function  &        0\%  &        4\%      &        1\%    \\
Unsupported Function or Type  &       64\%  &      53\%      &      59\%       \\
Unsupported Operation &                 1\% &    9\%   &       5\%    \\
Unsuccessful Setting &             0\%  &        4\%    &        1\%   \\
Misc                &             1\%  &         1\%     &        1\%    \\
\midrule
Timeout & 0 & 1 & 0 \\
Crash & 0& 2& 0\\
\bottomrule
\end{tabular}


==> assets/table/RQ4-SLT-demo-detailed.tex <==
\begin{tabular}{lrrrl}
\toprule
{} &  DuckDB &  PostgreSQL &  MySQL &                                             REASON \\
\midrule
Command &             1 &             1 &             0 &                  REINDEX statements are not supported \\
Command &             4 &             8 &             0 &                  REPLACE statements are not supported \\
Command &            23 &            23 &            23 &                 Trigger not supported or syntax error \\
Command &             0 &             0 &             1 &             "DROP INDEX index\_name" is not supported. \\
Function &             0 &           387 &             0 &                        CAST (as Integer) use round() \\
Function &             0 &           114 &             0 &    \texttt{CASE END} would cast all arguments and return value after casted \\
Function &             0 &            82 &             0 &    \texttt{COALESCE} Functions would cast all arguments and return value after casted \\
Function &             0 &            26 &             0 &    \texttt{NULLIF} Functions would cast all arguments and return value after casted \\
Function &        104033 &             0 &             0 &    In SQLite, '\textbackslash ' is used as the default symbol for integer division\\
Issue &             0 &             0 &             1 &                              Execution time is too long \\
Operation &          1278 &             0 &           832 &   A column is not included in the GROUP BY clause\\
Operation &             8 &             8 &             0 &               A non-empty set of values is required \\
Operation &          7075 &          6065 &             0 &   The unary plus'+' is not supported on a text type in target DBMS \\
Operation &             3 &             3 &             0 &               Multiple values updates not supported \\
Operation &             0 &          4860 &             0 &                        Depedencies on other objects \\
Operation &             0 &             4 &             0 &                                   Invalid type cast \\
Operation &             0 &             2 &             2 &    Performing update and delete operations on views \\
Operation &            43 &            12 &             0 &                                    Integer overflow \\
\bottomrule
\end{tabular}



==> assets/table/RQ4-SLT.tex <==
\begin{tabular}{lrrrrrrrrr}
    \toprule
        & \multicolumn{3}{c}{SQL Logic Test} \\               
    {}              &  DuckDB &  PostgreSQL &  MySQL  \\      
    \midrule
    Unsupported SQL statement           & 1,317 & 4,905 & 915\\      
    Inconsistent function \& operator              & 104,033   & 609 & 0 \\    
    Unsupported function                & 0  & 0 & 0 \\       
    Unsupported type                    & 43  & 12 & 0 \\     
    Unsupported operator                & 7,075 & 6,069 & 0 \\  
    Unknown system setting              &  0 & 0 & 0 \\       
    \midrule
    Timeout                             & 0      & 0      & 1  \\
    \bottomrule
\end{tabular}

==> assets/table/RQ4-compatibility.tex <==
\begin{table*}[tb]
\centering
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Issues} & \textbf{SQLite} & \textbf{MySQL} & \textbf{PostgreSQL} & \textbf{DuckDB} \\
\midrule
'\textbackslash' is used as default symbol for integer division & $\checkmark$ & X & $\checkmark$&  X\\
\midrule
CAST (as Integer) use round() & X & $\checkmark$& $\checkmark$ & $\checkmark$ \\
\midrule
Typecast all arguments for \texttt{COALESCE} & X & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
\midrule
Typecast all arguments for control flow functions & X & X & $\checkmark$ & X \\
\bottomrule
\end{tabular}
\caption{Compatibility Issues That Could Cause Query Results Difference}
\label{table:RQ4-compatibility}
\end{table*}

==> assets/table/RQ4-exp-setup.tex <==
\centering
\caption{DBMS experimental setup for cross-DBMS execution}\label{table:suties}
\begin{tabular}{ lrr }
\toprule
DBMS & Engine & Test Suite  \\ 
Names & Version & Version \\ 
\midrule
SQLite & 3.41.1 & \texttt{a22803} \\ 
PostgreSQL & 15.2 & \texttt{bc9993} \\
DuckDB & 0.8.2 & \texttt{49f21b}\\ 
MySQL & 8.0.33 & -  \\ 
\bottomrule
\end{tabular}

==> assets/table/RQ4-overall.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
    & \multicolumn{3}{c}{SQL Logic Test} &  \multicolumn{3}{c}{DuckDB Test Suite} & \multicolumn{3}{c}{PostgreSQL Test Suite}  \\
{}              &  DuckDB &  PostgreSQL &  MySQL  &  SQLite &  PostgreSQL &  MySQL  &  SQLite &  DuckDB &  MySQL  \\
\midrule
Unsupported SQL statement            & 28 & 32 & 24& 14\%  &     21\%       &        14\%    &  34\%   & 29\%   & 32\%  \\
Inconsistent function               & 0   & 609 & 0 &     1\%  &       4\%     &        1\%    &  0\%    & 4\%    & 1\%   \\
Unsupported function                & 0  & 0 & 0 &    67\%  &      61\%      &         62\%     &  64\%   & 53\%   & 59\%  \\
Unsupported type                    & 7,118  & 6,081 & 0 &    67\%  &      61\%      &         62\%     &  64\%   & 53\%   & 59\%  \\
Unsupported operator                & 104,033 & 0 & 0 &  18\% &     11\%    &        21\%   &  1\%    & 9\%    & 5\%   \\
Unknown system setting              &  0 & 0 & 0 &  0\%  &      2\%        &        1\%    &  0\%    & 4\%    & 1\%   \\
Misc                                & 1,289 & 4,873 & 891 &  0\%  &        1\%       &         0\%   &  1\%    & 1\%    & 1\%   \\ 
\midrule
Timeout                      & 0      & 0      & 1  & 0      & 0      & 0 & 0      & 1      & 0    \\
Crash                        & 0      & 0      & 0  & 0      & 1      & 0  & 0      & 2      & 0   \\ 
\bottomrule
\end{tabular}


==> assets/table/TestRunners.tex <==
\centering
\caption{Information of DBMS Test Runners}\label{table:runners}
\begin{tabular}{ lllll }
\toprule
DBMS & Test & Test & Result & Test & Test\\ 
Names & Content & Schedule & Validation & Client & Server\\ 
\midrule
SQLite & SQL & Separated & Record like & ODBC & N.A.\\ 
MySQL & Mostly SQL & TBA & File-like & TBA & TBA\\ 
PostgreSQL & Mostly SQL & Plan & All together & PSQL & Build from source\\ 
CockroachDB & SQL & Separated & Record like & TBA & TBA\\ 
DuckDB & SQL & Separated & Record like & CLI & N.A.\\ 
\bottomrule
\end{tabular}

==> assets/table/TestSuitesTable.tex <==
\centering
\caption{DBMS rankings and their test suites information}\label{table:suties}
\begin{tabular}{ lrrrrr }
\toprule
DBMS & DB-Engines & GitHub & Test & Runner\\ 
Names & Rankings & Stars & Files & LOC\\ 
\midrule
SQLite & 10 & 3.2k & 622& 10K\\ 
MySQL & 2 & 8.5k & 1413 & 20K\\ 
PostgreSQL & 4 & 11.3k & 212 & 3.5K \\
DuckDB & 171 & 7.4k & 2537 & 3K\\ 
\bottomrule
\end{tabular}

==> assets/table/TestSuitesTableFilter.tex <==
\centering
\caption{Test Suites Information after Filtering}\label{table:suties_filter}
\begin{tabular}{ lrrrr }
\toprule
DBMS &  Filter & Original & Current & Current \\ 
Names & Files & Files & Files & Test Cases \\ 
\midrule
SQLite & - & - & - & -\\ 
MySQL & - & - & - & -\\ 
PostgreSQL & - & - & - & -\\ 
CockroachDB & - & - & - & -\\ 
DuckDB & - & - & - & -\\ 
\bottomrule
\end{tabular}

==> assets/table/postgresql_error_analysis.tex <==
\begin{table}
\centering
\caption{Number of errors for each reason}
\label{tab:postgresql-error-reasons}
\begin{tabular}{lrrr}
\toprule
{} & sqlite & psql &  mysql \\
\midrule
ALREADYEXIST &    100 &    4 &     47 \\
COLLATION    &    203 &   47 &    208 \\
DEP-DDL      &   2338 &   18 &   2413 \\
DEP-DML      &    519 &    2 &    246 \\
DEP-EXT      &   2065 &   37 &   1960 \\
FUNCFORMAT   &    141 &    1 &    664 \\
LARGEOBJ     &     60 &   16 &     47 \\
NOEXIST      &   1730 &  132 &   1813 \\
Other        &   1390 &   40 &   2349 \\
PREPARETXN   &     19 &   20 &     19 \\
SYNTAX       &  16919 &    0 &  17623 \\
TIMESTAMP    &    470 &   18 &    501 \\
REGRESS      &      0 &   15 &      0 \\
SHOWTABLE    &      0 &   88 &      0 \\
\bottomrule
\end{tabular}
\end{table}

